Exponential Low-Regularity Parareal Algorithms for Nonlinear Schr\"odinger Equations

The parareal algorithm is one of the most widely studied parallel-in-time methods for the numerical approximation of time-dependent problems. For non-diffusive equations, however, standard parareal methods may converge slowly or even become unstable due to the absence of damping, while nonlinear interactions can transfer and amplify phase errors across Fourier modes. In this work, we consider the nonlinear Schr\"odinger equation (NLS) as a representative non-diffusive model and analyze parareal algorithms with an exact fine propagator, with particular emphasis on the design of suitable coarse propagators. We establish a general convergence framework, valid for solutions with limited regularity, under stability and local truncation error assumptions on the coarse propagator. These assumptions are verified for selected exponential low-regularity integrators designed for one-dimensional quadratic and cubic NLS equations, which achieve optimal approximation orders without derivative loss. To the best of our knowledge, this is the first construction of parareal algorithms for NLS equations that are provably linearly convergent, with a contraction factor proportional to the coarse time-step size even for solutions of limited regularity. Numerical experiments on quadratic, cubic, and quintic NLS equations demonstrate rapid convergence and improved performance over parareal variants using classical coarse propagators, including Lie and Strang splitting methods and first- and third-order exponential Runge--Kutta integrators.

==> environment.tex <==

% 引入所需的宏包
\usepackage[notref,notcite]{showkeys} % To see crossreferences.
\usepackage{braket,amsfonts}
\usepackage{amsmath,amssymb,amsxtra}
\usepackage{bm,mathrsfs,marvosym,eurosym}
\usepackage{mathtools,enumerate}
\usepackage{caption}
\usepackage{booktabs}
\usepackage{threeparttable}
\usepackage{comment}
\usepackage{nccmath}
\usepackage{bbm}
\usepackage{array}
\usepackage{multirow}
\usepackage{subcaption} 
\usepackage[normalem]{ulem}
\usepackage{upgreek}
\usepackage{tikz}
\usetikzlibrary{arrows,calc,decorations.pathreplacing}
\usetikzlibrary{arrows.meta, positioning}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{hyperref}

\setlength{\textwidth}{145mm}
% 创建数学运算符
\DeclareMathOperator*{\argmax}{argmax}
\def\d{{\mathrm d}}

\def\D{\mathscr{D}}
\def\G{\mathcal{G}}
\def\F{\mathcal{F}}
\def\U{{\mathcal U}}
\def\V{{\mathcal V}}

\def\R{{\mathcal R}}
\def\p{{\P}}
\def\P{{\mathcal P}}
\def\eps{\varepsilon}
\def\u{\mathbf{u}}

\def\A{{\mathcal{A}}}
\def\H{{\mathcal{H}}}
\def\B{{\mathcal{B}}}
\def\I{{\mathcal{I}}}
\def\Para{{{\large\textsc{Parareal}}}}
\def\0{{\textbf{0}}}

\def\l{\ell }
\def \a{\alpha }
\def \b{\beta }
\def \g{\gamma }
\def \L{\mathcal{L}}
\def \t{\theta}
\def\u{\mathbf{u}}
\def\w{\mathbf{w}}
\def\U{\mathbf{U}}
\def\E{\mathbf{E}}
\def \lam{\lambda}
\def\gl{\gamma_\mathrm{lin}}

\def \bA{\textbf{A}}
\def \fy{\varphi}
\def\<{{\langle }}
\def\>{{\rangle }}

\def\wU{\widehat U}
\def\wR{\widehat R}
\def\he{\hat e}
\def\Dom{\text{Dom}}
\def\II{(\Omega)}

\definecolor{darkred}{RGB}{200,0,0}
\definecolor{darkblue}{RGB}{0,0,200}
\definecolor{darkgreen}{RGB}{0,160,0}

% SIAM Shared Information Template
\usepackage{lipsum}

% 定义新的 theorem 环境
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}

\newcommand{\Tau}{\bm{\tau}}
\newtheorem{example}{\textit{Example}}

\newtheorem{assumption}{\textit{Assumption}}

%% Added on Overleaf: enabling xr
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}% latexmk will find this if $recorder=0 (however, in that case, it will ignore #1 if it is a .aux or .pdf file etc and it exists! if it doesn't exist, it will appear in the list of dependents regardless)
  \@addtofilelist{#1}% if you want it to appear in \listfiles, not really necessary and latexmk doesn't use this
  \IfFileExists{#1}{}{\typeout{No file #1.}}% latexmk will find this message if #1 doesn't exist (yet)
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}
% 设置标题和作者信息
\title{Exponential Low-regularity Parareal Algorithms for  Nonlinear Schr\"{o}dinger Equations\thanks{The work  supported by National Natural Science Foundation of China (Project 12422117),
Hong Kong Research Grants Council (15302323) and an internal grant of Hong Kong Polytechnic University (Project ID: P0053938, Work Programme: 4-ZZVA).}}
\author{ 
Qingle Lin\thanks{Department of Applied Mathematics, The Hong Kong Polytechnic University, Kowloon, Hong Kong, P.R. China (\texttt{qingle.lin@connect.polyu.hk})}
\and Zhi Zhou\thanks{Department of Applied Mathematics, The Hong Kong Polytechnic University, Kowloon, Hong Kong, P.R. China (\texttt{zhizhou@polyu.edu.hk})}
}


% 设置页面头部信息
\headers{LOW-Regularity Parareal for NLS}{Q. Lin, and Z. Zhou}


==> environment1.tex <==

% 引入所需的宏包
\usepackage[notref,notcite]{showkeys} % To see crossreferences.
\usepackage{braket,amsfonts}
\usepackage{amsmath,amssymb,amsxtra}
\usepackage{bm,mathrsfs,marvosym,eurosym}
\usepackage{mathtools,enumerate}
\usepackage{caption}
\usepackage{booktabs}
\usepackage{threeparttable}
\usepackage{comment}
\usepackage{nccmath}
\usepackage{bbm}
\usepackage{array}
\usepackage{multirow}
\usepackage{subcaption} 
\usepackage[normalem]{ulem}
\usepackage{upgreek}
\usepackage{tikz}
\usetikzlibrary{arrows,calc,decorations.pathreplacing}
\usetikzlibrary{arrows.meta, positioning}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\makeatletter
\@ifpackageloaded{hyperref}{}{\usepackage{hyperref}}
\makeatother

%\setlength{\textwidth}{145mm}
% 创建数学运算符
\DeclareMathOperator*{\argmax}{argmax}
\def\d{{\mathrm d}}

\def\D{\mathscr{D}}
\def\G{\mathcal{G}}
\def\F{\mathcal{F}}
\def\U{{\mathcal U}}
\def\V{{\mathcal V}}

\def\R{{\mathcal R}}
\def\p{{\P}}
\def\P{{\mathcal P}}
\def\eps{\varepsilon}
\def\u{\mathbf{u}}

\def\A{{\mathcal{A}}}
\def\H{{\mathcal{H}}}
\def\B{{\mathcal{B}}}
\def\I{{\mathcal{I}}}
\def\Para{{{\large\textsc{Parareal}}}}
\def\0{{\textbf{0}}}

\def\l{\ell }
\def \a{\alpha }
\def \b{\beta }
\def \g{\gamma }
\def \L{\mathcal{L}}
\def \t{\theta}
\def\u{\mathbf{u}}
\def\w{\mathbf{w}}
\def\U{\mathbf{U}}
\def\E{\mathbf{E}}
\def \lam{\lambda}
\def\gl{\gamma_\mathrm{lin}}

\def \bA{\textbf{A}}
\def \fy{\varphi}
\def\<{{\langle }}
\def\>{{\rangle }}

\def\wU{\widehat U}
\def\wR{\widehat R}
\def\he{\hat e}
\def\Dom{\text{Dom}}
\def\II{(\Omega)}

\definecolor{darkred}{RGB}{200,0,0}
\definecolor{darkblue}{RGB}{0,0,200}
\definecolor{darkgreen}{RGB}{0,160,0}

% 定义新的 theorem 环境
\makeatletter
\@ifundefined{newsiamremark}{%
  \newtheorem{theorem}{Theorem}[section]
  \newtheorem{lemma}{Lemma}[section]
  \newtheorem{remark}{Remark}[section]
  \newtheorem{example}{Example}[section]
  \newtheorem{proposition}{Proposition}[section]
  \newtheorem{corollary}{Corollary}[section]
  \newtheorem{assumption}{Assumption}[section]
  \newtheorem{claim}{Claim}[section]
  \providecommand{\headers}[2]{}
  \@ifundefined{keywords}{%
    \newenvironment{keywords}{\vskip5pt\noindent\textbf{Keywords}: }{\par}%
  }{}%
}{%
  \newsiamremark{remark}{Remark}
  \newsiamremark{hypothesis}{Hypothesis}
  \@ifundefined{crefname}{}{\crefname{hypothesis}{Hypothesis}{Hypotheses}}
  \newsiamthm{claim}{Claim}
  \newtheorem{example}{\textit{Example}}
  \newtheorem{assumption}{\textit{Assumption}}
}
\makeatother

\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}

\newcommand{\Tau}{\bm{\tau}}


%% Added on Overleaf: enabling xr
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}% latexmk will find this if $recorder=0 (however, in that case, it will ignore #1 if it is a .aux or .pdf file etc and it exists! if it doesn't exist, it will appear in the list of dependents regardless)
  \@addtofilelist{#1}% if you want it to appear in \listfiles, not really necessary and latexmk doesn't use this
  \IfFileExists{#1}{}{\typeout{No file #1.}}% latexmk will find this message if #1 doesn't exist (yet)
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}
% 设置标题和作者信息
\title{Exponential Low-regularity Parareal Algorithms for  Nonlinear Schr\"{o}dinger Equations\thanks{The work  supported by National Natural Science Foundation of China (Project 12422117),
Hong Kong Research Grants Council (15302323) and an internal grant of Hong Kong Polytechnic University (Project ID: P0053938, Work Programme: 4-ZZVA).}}
\author{ 
Qingle Lin\thanks{Department of Applied Mathematics, The Hong Kong Polytechnic University, Kowloon, Hong Kong, P.R. China (\texttt{qingle.lin@connect.polyu.hk})}
\and Zhi Zhou\thanks{Department of Applied Mathematics, The Hong Kong Polytechnic University, Kowloon, Hong Kong, P.R. China (\texttt{zhizhou@polyu.edu.hk})}
}


% 设置页面头部信息
\headers{LOW-Regularity Parareal for NLS}{Q. Lin, and Z. Zhou}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}
